Double Descent and Overfitting under Noisy Inputs and Distribution Shift for Linear Denoisers

Despite the importance of denoising in modern machine learning and ample empirical work on supervised denoising, its theoretical understanding is still relatively scarce. One concern about studying supervised denoising is that one might not always have noiseless training data from the test distribution. It is more reasonable to have access to noiseless training data from a different dataset than the test dataset. Motivated by this, we study supervised denoising and noisy-input regression under distribution shift. We add three considerations to increase the applicability of our theoretical insights to real-life data and modern machine learning. First, while most past theoretical work assumes that the data covariance matrix is full-rank and well-conditioned, empirical studies have shown that real-life data is approximately low-rank. Thus, we assume that our data matrices are low-rank. Second, we drop independence assumptions on our data. Third, the rise in computational power and dimensionality of data have made it important to study non-classical regimes of learning. Thus, we work in the non-classical proportional regime, where data dimension $d$ and number of samples $N$ grow as $d/N = c + o(1)$. For this setting, we derive data-dependent, instance specific expressions for the test error for both denoising and noisy-input regression, and study when overfitting the noise is benign, tempered or catastrophic. We show that the test error exhibits double descent under general distribution shift, providing insights for data augmentation and the role of noise as an implicit regularizer. We also perform experiments using real-life data, where we match the theoretical predictions with under 1\% MSE error for low-rank data.

==> introduction.tex <==
\section{Introduction}

Denoising and noisy-input problems have a rich history in machine learning and signal processing [cite Baldi and Hornik, future denoising papers, noisy input papers], and it is well understood that non-trivial denoising is made possible by the presence of additional structure in the data [cite autoencoder papers]. One of the most natural such structures is the true inputs being low-rank \rishi{maybe we say lives in low-dim linear subspace}. In fact, past work from [cite low rank works] has demonstrated that a lot of real-life data is low-rank -- that is, its covariance matrix only has a few significant eigenvalues. 

% We will discuss below that while this intuition has helped make progress in unsupervised settings, little is known about supervised settings, especially in modern non-classical data regimes \rishi{This sentence confuses me}. Here the analysis is highly non-trivial, further complicated by incorporating distribution shift and dropping IID assumptions.


While significant progress has been made in the theoretical and empirical understanding of unsupervised denoising \ck{unsupervised methods for denoising, such as PCA, low rank matric recovery} \rishi{What is unsupervised denoising?} [cite PCA again] by leveraging this intuition, little is known about non-trivial phenomena in supervised denoising and noisy-input problems. 

One of the biggest practical qualms to considering a supervised setting is that a learner needs access to noiseless data sampled from the test distribution. However, this is resolved by considering distribution shift, which is when the training and test data can come from different distributions. One often has access to noiseless data of the same \textit{nature} as the test dataset, but generated by a potentially different data distribution. One can add noise to such data to train an effective denoising or regression function in a supervised fashion. As a toy example, one might have access to noiseless dog pictures containing mostly German shepherds and collies, but would want to denoise noisy dog pictures containing mostly pomeranians and poodles. As long as the training data ``spans" the approximate low-rank subspace containing dog pictures, meaningful learning is possible. The same argument can be made for regression with noisy inputs, say for predicting click-rates for these pictures. Given this practical motivation, we study supervised noisy-input problems under distribution shift. \rishi{I really like this paragraph}


\rishi{I think we need another paragraph on theory work.}

The classical version of such problems would keep the data dimension $d$ fixed and let the number of samples $N$ grow to $\infty$. These can be theoretically analysed using elementary tools. However, with growing access to computational power and richness of data, it has become important to study non-classical data regimes, such as when $d$ and $N$ grow proportionally [cite stuff]. Phenomena like double-descent and benign overfitting in \textit{noiseless} input settings demonstrate the surprising advantages of high dimensionality. \ck{remove next sentence, emphasize that we don't need anything to go to $\infty$ and we give error bounds} As argued in \cite{cheng2022dimension}, the non-classical regime is the proportional regime, where $d, N \to \infty$ and $d/N \to c>0$. However, there is very little work on learning with \textit{noisy} inputs in this regime. Our paper takes one of the first steps towards filling this gap by studying supervised noisy-input problems in the proportional regime. Following the trend of past theoretical work in noiseless input settings, we start by considering the fundamental problem of learning linear functions. \rishi{This one is confusing. Specially since our experiments don't scale $d$. I think, we need to phrase our results as true in general. Maybe we present it as a bound. That is error - our estimate is bounded by by our error term, which seems to decay. }

However, most past theoretical work in the noiseless input setting does not test on or performs poorly on real-life data. As argued above and in \cite{cheng2022dimension}, a big reason for this issue is that past work assumes that the data covariance matrix is well-conditioned, while real-life data covariance matrices are better modeled by low-rank assumptions. We aim to address this issue by testing our theory for low-rank data on real-life datasets. 

In real life, one has little control over the independence or even the distribution of the data [find citations]. We would thus like to work with non-IID data in a distribution-free manner -- that is, without any assumptions on the structure of the data distribution. Additionally, explicit structural assumptions made about distribution shift in past work are often quite restrictive, and involve the joint distribution of training and test data [find citations showing they are restrictive]. We would like to work without such assumptions. In summary, we aim to address the following question:

\begin{center}
    \textit{Can we derive test error expressions for linear denoising and regression with noisy inputs on non-IID low-rank data in the proportional regime that are (1) distribution-free, (2) free of structural assumptions on the distribution shift, (3) match experiments on real-life data?\\ What insights can we obtain from these?}
\end{center}

\paragraph{Contributions and Paper Structure.} 
% Given low-dimensional data $x_i$, embedded in high-dimensional space, we add noise to $x_i$ to get a noisy version $y_i$. Then, we are interested in finding the linear denoiser $W$ that minimizes the least squares problem, 
% \[
% \sum_{i} \|x_i - Wy_i\|_2^2.
% \]
% For this setup, Theorem \ref{thm:main} provides the generalization error \emph{without} needing assumptions involving the independence or identical distribution of \emph{either the training or test data}. The paper \emph{decouples assumptions on the training and test distribution}. This lets us also address the problem of distributional shift. Crucially, this means that Theorem 1 applies to various scenarios. We highlight this using the applications mentioned in Table \ref{tab:my_label}. We further show a strong correlation between the in-distribution and out-of-distribution risks by bounding the difference between the two risks by a quantity independent of the training data. We show that increasing the over-parameterization \cite{covariateNew} or increasing the amount of \emph{in-distribution} training data points moves us away from the peak of the generalization error curve, which improves \emph{both in-distribution and out-of-distribution} generalization errors by the previous conclusion. 


\rishi{Maybe we could move contributions to post related work? That way it might help with the comments that we don't properly put our results in context.}

The major contributions of the paper are as follows.
\begin{enumerate}[nosep]
    \item (\textbf{Distribution-Free Expressions Without IID Assumptions}) We derive test error expressions (Theorem \ref{thm:main}, \ref{thm:transfer}) for linear denoising and regression with noisy inputs, without IID assumptions on the low-rank data and in a distribution-free manner.
    \item (\textbf{General Distribution Shift}) Unlike most prior work on distribution shift, we do not need assumptions on the joint distribution of training and test data for test error guarantees. We bound the difference between in-distribution and out-of-distribution expected risk in a distribution-free manner (Theorem \ref{prop:in-out-dist}, Corollary \ref{cor:bound-out-of-subspace}). 
    \item (\textbf{Data Augmentation Insights}) We examine when data augmentation improves both in-distribution and out-of-distribution generalization, giving theoretical results and practical insights (Corollary \ref{cor:data-augmentation}).  
    \item (\textbf{Real Data Experiments}) We test on real data and get a relative error of under 1\%, establishing that our theoretical results can be used with real data.\footnote{The code for the experiments can be found in the following anonymized repository \href{https://anonymous.4open.science/r/Low-Rank-Generalization-Without-IID-99F7/README.md}{[Link]}.} 
\end{enumerate}

Section \ref{sec:setup} provides details and theoretical assumptions for the model we analyze. Section \ref{sec:main} discusses our main theoretical results for the denoising problem. Section \ref{sec:app} discusses applications of the result to data augmentation, linear regression, and a specific instantiation of our results if we assume the test data is I.I.D. 

\subsection{Related Work}

\paragraph{Denoising.} [ADD STUFF]

\paragraph{Linear Regression.} There has been significant work in understanding the generalization error for linear regression \cite{sonthalia2023training, Dobriban2015HighDimensionalAO, pmlr-v139-mel21a, Muthukumar2019HarmlessIO, Bartlett2020BenignOI, Belkin2020TwoMO, Derezinski2020ExactEF, Hastie2019SurprisesIH, loureiro2021learning} and kernelized regression \cite{MEI20223, Mei2021TheGE, Mei2018AMF, Tripuraneni2021CovariateSI, pmlr-v119-gerace20a, pmlr-v125-woodworth20a, Loureiro2021LearningCO, NEURIPS2019_c133fb1b, NEURIPS2020_a9df2255}. While our work benefits from their insights and techniques, our introduction and \cite{cheng2022dimension} outline issues in applying their theory to real data, which violates their IID and full-rank well-conditioning assumptions. The latter issue is partially addressed by work on Principal Component Regression \cite{teresa2022, xu2019number}. %These works use a PCA-based low-rank approximation of the data and provide theoretical results in terms of the effective rank or eigenvalue decay of the data covariance matrix. 
However, they do not test on real data. 

\paragraph{Testing on Real-Life Data.} Some past theoretical work tests on real data \cite{loureiro2021learning, Loureiro2021LearningCO, wei2022more}. 
%The first of these \cite{loureiro2021learning} assumes that the data distribution is given by a Gaussian mixture model. \cite{Loureiro2021LearningCO} uses a Gaussian equivalence principle to argue that their teacher-student model can capture realistic data assumptions. Finally, \cite{wei2022more} show that their appropriately rescaled training error asymptotically converges to the true risk under some assumptions. 
However, \emph{all} of these works require that the training data is \emph{I.I.D.} and that the test data is from the \emph{same distribution} as the training data, both of which contribute to mismatch between theory and experiments.

\paragraph{OOD Generalization and Distribution Shift.} Empirically, studies such as \cite{miller2021accuracy, recht2019imagenet, miller2020effect, mccoy-etal-2020-berts} have noticed that there is a strong linear correlation between in-distribution accuracy and out-of-distribution accuracy. There has been some theoretical work \cite{Tripuraneni2021CovariateSI,covariateNew,mania2020classifier, Darestani2021MeasuringRI,lejeune2022monotonic} that has looked into this phenomenon, but a general, concrete theory is still lacking. For example, both \cite{Tripuraneni2021CovariateSI} and \cite{wu2020optimal} need joint assumptions on the spectrum of the training and test data covariances. In other examples, \cite{NIPS2006_b1b0432c} approaches this from a domain adaptation perspective and compute bounds dependent on an abstract notion of distribution distance; \cite{pmlr-v139-lei21a} provides analysis for the minimax risk; and \cite{Lampinen2019AnAT} studies the generalization when training models with gradient descent.

% There has been some theoretical work \cite{Tripuraneni2021CovariateSI,covariateNew,mania2020classifier, Darestani2021MeasuringRI,lejeune2022monotonic} that has looked into this phenomenon, but a general theory is still lacking. For example, both \cite{Tripuraneni2021CovariateSI} and \cite{wu2020optimal} need joint assumptions on the spectrum of the training and test data covariances. There  \cite{NIPS2006_b1b0432c} that computes bounds on the VC dimension, \cite{pmlr-v139-lei21a} that provides analysis for the minimax risk, and \cite{Lampinen2019AnAT} that studies the generalization when training models with gradient descent.

\paragraph{Double Descent and Other Related Work.} [NEEDS EXPANSION/SPLITTING] The generalization curves in our paper display double descent \cite{opper1996statistical, Belkin2019ReconcilingMM}, which is believed to occur due to the implicit bias of the learning algorithms. There has been significant theoretical work on understanding implicit biases \cite{Ali2020TheIR, pmlr-v119-jacot20a, pmlr-v178-shamir22a, Neyshabur2017ImplicitRI, NIPS2017_10ce03a1, Neyshabur2015InSO} and gradient descent \cite{Soudry2018TheIB, Lyu2020GradientDM,pmlr-v99-ji19a,bowman2022implicit, Chizat2020ImplicitBO, du2019gradient, du2018gradient, Ali2019ACV, Paquette2022ImplicitRO, Poole2016, 10.5555/3546258.3546283, Paquette2022HomogenizationOS}. 

\begin{table}[!ht]
\setlength{\tabcolsep}{3pt}
    \caption{Table with common assumptions for theoretical work and common application domains for the results. A model is well specified if the target function being modeled is within the class of functions the model can represent.}
    \label{tab:my_label}
    \centering
    \renewcommand{\arraystretch}{0}
    \begin{tabular}{ccccc|cccccc|c}
        \toprule
        \multicolumn{5}{c}{Assumptions} & Ref. \\
       \makecell{Non-\\I.I.D.} & \makecell{Separate \\ train, test} & \makecell{Low-\\Rank} & \makecell{Norm\\Decay} & \makecell{Input\\Noise} & \\ \midrule
        \tikzxmark & \tikzxmark & \tikzxmark & \tikzxmarkgreen & \tikzxmark & \cite{Dobriban2015HighDimensionalAO,Bartlett2020BenignOI} \\
        \tikzxmark & \tikzxmark & \tikzxmark & \tikzxmarkgreen & \tikzxmark & \cite{Hastie2019SurprisesIH} \\
       \tikzxmark & \tikzxmark & \tikzxmark & \tikzxmarkgreen & \tikzxmark & \cite{Tripuraneni2021CovariateSI, covariateNew} \\
       \tikzxmark & \tikzxmark & \tikzxmark & \tikzxmarkgreen & \tikzxmark & \cite{Loureiro2021LearningCO,wei2022more} \\
       \tikzxmark & \tikzxmark & \checkmark & \tikzxmarkgreen & \tikzxmark & \cite{loureiro2021learning} \\
       \tikzxmark & \tikzxmark & \checkmark & \tikzxmarkgreen & \tikzxmark & \cite{teresa2022, xu2019number, wu2020optimal} \\
       \tikzxmark & \checkmark & \checkmark & \tikzxmarkgreen & \checkmark & \cite{sonthalia2023training,sonthaliaUnderPeak} \\
       \checkmark & \checkmark & \checkmark & \checkmarkred\tablefootnote{Only for over-parameterized models} & \checkmark & This paper \\ \bottomrule
    \end{tabular}
\end{table}


